Privacy Threats in Stable Diffusion Models

This paper introduces a novel approach to membership inference attacks (MIA) targeting stable diffusion computer vision models, specifically focusing on the highly sophisticated Stable Diffusion V2 by StabilityAI. MIAs aim to extract sensitive information about a model's training data, posing significant privacy concerns. Despite its advancements in image synthesis, our research reveals privacy vulnerabilities in the stable diffusion models' outputs. Exploiting this information, we devise a black-box MIA that only needs to query the victim model repeatedly. Our methodology involves observing the output of a stable diffusion model at different generative epochs and training a classification model to distinguish when a series of intermediates originated from a training sample or not. We propose numerous ways to measure the membership features and discuss what works best. The attack's efficacy is assessed using the ROC AUC method, demonstrating a 60\% success rate in inferring membership information. This paper contributes to the growing body of research on privacy and security in machine learning, highlighting the need for robust defenses against MIAs. Our findings prompt a reevaluation of the privacy implications of stable diffusion models, urging practitioners and developers to implement enhanced security measures to safeguard against such attacks.

==> assets/features_compared.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{assets//images/metrics_progression.pdf}
    \caption{Visual representation of vector features produced by two example encoders. On the top are three member and three non-member images, whose features are encoded using the PSNR metric (\Cref{sec:psnr}) and the progress-based observer (\Cref{sec:progress_observer}). On the bottom are an equal number of members and non-members, processed using Euclidean distance between their encoded representations (\Cref{sec:euclid}) and also a progress-based observer. From a visual inspection alone, the samples are not easily distinguishable, and other samples we manually observed and did not include here are similar. A binary classifier, however, is able to pick up differences hidden to the naked eye.}
    \label{fig:features_compared}
\end{figure}

==> assets/one-shot_distribution.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{assets//images/one-shot_distribution.pdf}
    \caption{Comparison of the distributions of members vs non-members encoded features in a fully black-box setting. Different rows show different distance functions, and in all cases, the observer is One-Shot (see \Cref{sec:one-shot_observer}). The left column shows distributions for untouched images, whereas on the right the images are smoothed with box blurring of unit radius (producing a 3x3 box).}
    \label{fig:one-shot_distribution}
\end{figure*}
